Multimodal Large Language Models for Low-Resource Languages: A Case Study for Basque

Current Multimodal Large Language Models exhibit very strong performance for several demanding tasks. While commercial MLLMs deliver acceptable performance in low-resource languages, comparable results remain unattained within the open science community. In this paper, we aim to develop a strong MLLM for a low-resource language, namely Basque. For that purpose, we develop our own training and evaluation image-text datasets. Using two different Large Language Models as backbones, the Llama-3.1-Instruct model and a Basque-adapted variant called Latxa, we explore several data mixtures for training. We show that: i) low ratios of Basque multimodal data (around 20%) are already enough to obtain solid results on Basque benchmarks, and ii) contrary to expected, a Basque instructed backbone LLM is not required to obtain a strong MLLM in Basque. Our results pave the way to develop MLLMs for other low-resource languages by openly releasing our resources.

==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/agreementBenchmark.tex <==
\begin{table*}[t!]
\centering
\begingroup
\renewcommand{\arraystretch}{1.5} %
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \textbf{Acceptance Rate} & \textbf{Agreement} \\  %
\midrule
\rowcolor{gray!20}
VQAv2\textsubscript{Eus} & 0.8375 & 0.887 \\
Pixmo-CapQA\textsubscript{Eus} & 0.8625 & 0.887 \\                                  %
\rowcolor{gray!20}
A-OKVQA\textsubscript{Eus}  & 0.975  & 0.95 \\                                  %
\bottomrule
\end{tabular}
\endgroup
\caption{Sample acceptance rate and mean inter-annotator agreement between the 4 annotators. The agreement has been calculated by using 40 images.}
\label{eval:eval_data_annotation}
\end{table*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/architecture.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/architectureIm.pdf}
    \caption{The late-fusion MLLM architecture used in this work. Our MLLMs have a visual encoder to represent input images, a connector to project visual representations into the embedding space of the LLM, and an LLM to process image inputs and textual queries to generate textual answers.}
    \label{fig:architecture}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/judmentTable.tex <==



\begin{table*}[t!]
\centering
\small
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{3}{c}{\textbf{Human}} & \multicolumn{3}{c}{\textbf{GPT-5}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \textbf{Latxa} & \textbf{Tie} & \textbf{Llama} & \textbf{Latxa} & \textbf{Tie} & \textbf{Llama} \\
\midrule
\textbf{Winning \%} & 23.11 & 53.79 & 20.45 & 31.44 & 36.74 & 31.82· \\
\bottomrule
\end{tabular}
\caption{Multimodal open-ended performance comparison between top-performing Llama-based and Latxa-based MLLMs across human and automated evaluation paradigms. Human evaluations resulted in inconclusive outcomes for 3\% of samples due to annotation discrepancies.}
\label{tb:human_annotation}
\end{table*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/multimodalEmaitzak.tex <==
\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\begin{axis}[
hide axis,
xmin=0, xmax=1,
ymin=0, ymax=1,
width=2cm,
height=2.5cm,
legend style={
at={(0.5,0.5)},
anchor=center,
legend columns=2,
/tikz/every even column/.append style={column sep=1cm}
},
]`
\addlegendimage{line width=1.5pt, color=red!60, mark=, mark options={fill=red!60, scale=0.8}}
\addlegendentry{English}
\addlegendimage{line width=1.5pt, color=blue!60, mark=, mark options={fill=blue!60, scale=0.8}}
\addlegendentry{Basque (translated)}
\end{axis}
\end{tikzpicture}
\vspace{0.3cm}

\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    ylabel={Performance},
    ylabel near ticks,
    title={VQAv2},
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.62) (20, 0.63) (80, 0.61) (100, 0.05)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.45) (20, 0.59) (80, 0.62) (100, 0.61)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    title={A-OKVQA},
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.59) (20, 0.63) (80, 0.63) (100, 0.59)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.50) (20, 0.55) (80, 0.59) (100, 0.52)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    title={PixMoCapQA},
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.66) (20, 0.69) (80, 0.69) (100, 0.70)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.51) (20, 0.54) (80, 0.55) (100, 0.51)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{tikzpicture}[overlay, remember picture]
\fill[purple!35!white] (0.1, 0.5) rectangle (0.7, 2.9);
\node[rotate=90, anchor=center] at (0.4, 1.8) {\large \textbf{Latxa}};
\end{tikzpicture}

\vspace{0.7cm}

\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Basque Multimodal Data \%},
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    xlabel near ticks,
    ylabel={Performance},
    ylabel near ticks,
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.62) (20, 0.63) (80, 0.58) (100, 0.08)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.24) (20, 0.56) (80, 0.59) (100, 0.59)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Basque Multimodal Data \%},
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    xlabel near ticks,
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.54) (20, 0.63) (80, 0.65) (100, 0.62)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.35) (20, 0.51) (80, 0.58) (100, 0.58)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Basque Multimodal Data \%},
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=5.5cm,
    height=4.0cm,
    xlabel near ticks,
]
\addplot[line width=1.5pt, color=red!60, mark=*, mark options={fill=red!60, scale=0.8}] coordinates {
    (0, 0.72) (20, 0.69) (80, 0.71) (100, 0.70)
};
\addplot[line width=1.5pt, color=blue!60, mark=*, mark options={fill=blue!60, scale=0.8}] coordinates {
    (0, 0.51) (20, 0.54) (80, 0.52) (100, 0.61)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{tikzpicture}[overlay, remember picture]
\fill[blue!35!white] (0.1, 1.1) rectangle (0.7, 3.5);
\node[rotate=90, anchor=center] at (0.4, 2.3) {\large \textbf{Llama}};
\end{tikzpicture}

\caption{Accuracy across multimodal benchmarks of Latxa-based (top row) and Llama-based (bottom row) MLLMs trained with different percentages of Basque Multimodal Instruction Data. The models are evaluated on the English (original) and Basque (translated) versions of close-ended benchmarks. }
\label{fig:performance_benchmark_multimodal}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/prompts/translationAok.tex <==
\begin{figure*}[htbp]

\centering
\begin{tcolorbox}[
    colback=customblue!10,
    colframe=customblue,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Translation Procedure for \textbf{A-OKVQA\textsubscript{Eus}}: 2-Shot Prompting for English-Basque,
    width=0.95\textwidth]

\begin{tcolorbox}[
    colback=customblue!5,
    colframe=customblue!70,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=System Message,
    fonttitle=\bfseries]
\footnotesize
\textbf{Role:} System\\
\textbf{Content:} You are a helpful AI assistant that specializes in English to Basque translations.\textbackslash n Your task is to translate instruction datasets from English to Basque.\textbackslash n\textbackslash n Here are some important guidelines:\textbackslash n 1. Maintain the original meaning and intent of the instructions\textbackslash n 2. Use standard Basque language (batua)\textbackslash n 3. Keep technical terms that don't have widely accepted Basque translations\textbackslash n 4. Preserve any code snippets, variables, or special characters exactly as they appear\textbackslash n\textbackslash n Please provide accurate Basque translations for all text fields.
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 1,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answer to Basque \textbackslash n \textbf{Question}: What is the man by the bags awaiting? \textbackslash n \textbf{Answer}: 1.skateboarder, 2.train, 3.delivery, 4.cab

\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Zer ari da poltsekin dagoen gizona itxaroten?\textbf{Erantzuna:}  1.skaterra, 2.trena, 3.Deliveria, 4.Taxia
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 2,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} \textbf{Question:} Where does this man eat pizza? \textbf{Answer:} 1.office, 2.cafe, 3.motel, 4.outside
\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Non ari da gizon hau pizza jaten? \textbf{Erantzuna:} 1.Ofizinan, 2.Kafetegian, 3.Motelean, 4.Kanpoan
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!12,
    colframe=customblue!90,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=New Query,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answers to Basque \textbackslash n\textbackslash n\textbackslash n \textbf{Question}: \{example['question']\} \textbf{Answer}: \{example['answer']\}

\vspace{0.2cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} ... \textbackslash n \textbf{Erantzuna:} ...

\end{tcolorbox}

\end{tcolorbox}
\caption{Two-shot prompting procedure for English to Basque translation of the A-OKVQA\textsubscript{Eus} benchmark. {example['question']} and {example['answer']} correspond to the question and answer to be translated in the example. }
\label{fig:translation-procedure1}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/prompts/translationPix.tex <==
\begin{figure*}[htbp]

\centering
\begin{tcolorbox}[
    colback=customblue!10,
    colframe=customblue,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Translation Procedure for \textbf{PixMo-CapQA\textsubscript{Eus}}: 2-Shot Prompting for English-Basque,
    width=0.95\textwidth]

\begin{tcolorbox}[
    colback=customblue!5,
    colframe=customblue!70,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=System Message,
    fonttitle=\bfseries]
\footnotesize
\textbf{Role:} System\\
\textbf{Content:} You are a helpful AI assistant that specializes in English to Basque translations.\textbackslash n Your task is to translate instruction datasets from English to Basque.\textbackslash n\textbackslash n Here are some important guidelines:\textbackslash n 1. Maintain the original meaning and intent of the instructions\textbackslash n 2. Use standard Basque language (batua)\textbackslash n 3. Keep technical terms that don't have widely accepted Basque translations\textbackslash n 4. Preserve any code snippets, variables, or special characters exactly as they appear\textbackslash n\textbackslash n Please provide accurate Basque translations for all text fields.
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 1,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answer to Basque \textbackslash n \textbf{Question}: Is this room decorated for the 1970s?

\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Gela hau 1970ean bezala dago diseinatuta?
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 2,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answers to Basque \textbackslash n \textbf{Question:} Is there a mirror in the room?
\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Ba al dago ispilurik gelan?
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!12,
    colframe=customblue!90,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=New Query,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answers to Basque \textbackslash n\textbackslash n\textbackslash n \textbf{Question}: \{example['question']\} \textbf{Answer}: \{example['answer']\}

\vspace{0.2cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} ... \textbackslash n \textbf{Erantzuna:} ...

\end{tcolorbox}

\end{tcolorbox}
\caption{Two-shot prompting procedure for English to Basque translation of the PixMo-CapQA\textsubscript{Eus} benchmark. {example['question']} and {example['answer']} correspond to the question and answer to be translated in the example. }
\label{fig:translation-procedure2}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/prompts/translationVqa.tex <==
\begin{figure*}[htbp]

\centering
\begin{tcolorbox}[
    colback=customblue!10,
    colframe=customblue,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Translation Procedure for \textbf{VQAv2\textsubscript{Eus}}: 2-Shot Prompting for English-Basque,
    width=0.95\textwidth]

\begin{tcolorbox}[
    colback=customblue!5,
    colframe=customblue!70,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=System Message,
    fonttitle=\bfseries]
\footnotesize
\textbf{Role:} System\\
\textbf{Content:} You are a helpful AI assistant that specializes in English to Basque translations.\textbackslash n Your task is to translate instruction datasets from English to Basque.\textbackslash n\textbackslash n Here are some important guidelines:\textbackslash n 1. Maintain the original meaning and intent of the instructions\textbackslash n 2. Use standard Basque language (batua)\textbackslash n 3. Keep technical terms that don't have widely accepted Basque translations\textbackslash n 4. Preserve any code snippets, variables, or special characters exactly as they appear\textbackslash n\textbackslash n Please provide accurate Basque translations for all text fields.
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 1,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answer to Basque \textbackslash n \textbf{Question}: Explain the visual content of the image in great detail.\textbackslash n \textbf{Answer}: In this outdoor wedding photo, a bride wearing a beautiful white dress is posing on a park bench surrounded by a group of five men dressed in suits. The groomsmen are wearing pink ties, adding a pop of color to the scene. The group is standing around the bride, smiling and enjoying the special occasion as they pose for the picture.\textbackslash n \textbackslash n. In the background, there are potted plants which further enhance the ambiance of the park setting. The bench, on which the bride is seated, is located close to the center of the image.

\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Azaldu irudia zehaztasun askorekin. \textbf{Erantzuna:}  Ezkontzako argazki honetan, soineko zuri eder bat daraman emaztegaia parkeko banku batean dago, trajez jantzitako bost gizonez inguratuta. Neskameek gorbata arrosak daramatzate, eszenari kolorezko pop bat erantsiz. Taldea emaztegaiaren inguruan dago, irribarretsu, eta aukera bereziaz gozatzen dute koadrorako. Jarlekua, non emaztegaia eserita dagoen, irudiaren erditik hurbil dago.
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 2,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answers to Basque \textbackslash n \textbf{Question:} What website copyrighted the picture? \textbf{Answer:} 1.foodiebakercom, 2.foodiebakercom, 3.foodiebaker, 4.foodiebakercom, 5.foodiebakercom, 6.http://foodiebakercom, 7.foodiebakercom, 8.foodiebakercom, 9.foodiebakercom, 10.foodiebaker
\vspace{0.3cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} Zein webgunek du irudiaren copyrigheta? \textbf{Erantzuna:} 1.foodiebakercom, 2.foodiebakercom, 3.foodiebaker, 4.foodiebakercom, 5.foodiebakercom, 6.http://foodiebakercom, 7.foodiebakercom, 8.foodiebakercom, 9.foodiebakercom, 10.foodiebaker
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!12,
    colframe=customblue!90,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=New Query,
    fonttitle=\bfseries]

\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Translate the following question and answers to Basque \textbackslash n\textbackslash n\textbackslash n \textbf{Question}: \{example['question']\} \textbf{Answer}: \{example['answer']\}

\vspace{0.2cm}

\textbf{Role:} Assistant\\
\textbf{Content:} \textbf{Galdera:} ... \textbackslash n \textbf{Erantzuna:} ...

\end{tcolorbox}

\end{tcolorbox}
\caption{Two-shot prompting procedure for English to Basque translation of the VQAv2\textsubscript{Eus} benchmark. {example['question']} and {example['answer']} correspond to the question and answer to be translated in the example.}
\label{fig:translation-procedure3}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/prompts/translationWildvision.tex <==
\begin{figure*}[htbp]

\centering
\begin{tcolorbox}[
    colback=customblue!10,
    colframe=customblue,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Translation Procedure for \textbf{Wildvision\textsubscript{Eus}}: 2-Shot Prompting for English-Basque,
    width=0.95\textwidth]

\begin{tcolorbox}[
    colback=customblue!5,
    colframe=customblue!70,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=System Message,
    fonttitle=\bfseries]
\footnotesize
\textbf{Role:} System\\
\textbf{Content:} Cutting Knowledge Date: December 2023
Today Date: [2025-01-01]

You are a helpful assistant
\end{tcolorbox}

\vspace{0.3cm}

\begin{tcolorbox}[
    colback=customblue!8,
    colframe=customblue!80,
    boxrule=1pt,
    arc=3pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    title=Shot 1,
    fonttitle=\bfseries]
\footnotesize
\textbf{Role:} User\\
\textbf{Content:} Honako testu hau gaztelaniaz idatzita dago eta euskerara itzuli behar da. Itzulpena zehatza eta naturala izan behar da. Jarri ezazu bakarrik testua, ez egin erreferentziarik hau itzulpen bat denik.

\textbf{Gaztelaniazko testua:} example['question']

\textbf{Euskerazko itzulpena:}


\vspace{0.3cm}

\textbf{Role:} Assistant\\
example['answer']
\end{tcolorbox}
\end{tcolorbox}
\caption{Prompt for the Spanish to Basque translation of the Wildvision\textsubscript{Eus} benchmark. {example['question']} and {example['answer']} correspond to the question and answer to be translated in the example. We used a 0-shot strategy for open-ended settings. }
\label{fig:translation-procedure4}
\end{figure*}


==> vqnynthkpvktnfqvxdctydcphdxkcczj_arXiv/figures/textonlyEmaitzak.tex <==
\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\begin{axis}[
hide axis,
xmin=0, xmax=1,
ymin=0, ymax=1,
width=10cm,
height=2.5cm,
legend style={
at={(0.5,0.5)},
anchor=center,
legend columns=3,
/tikz/every even column/.append style={column sep=1cm}
},
]
\addlegendimage{line width=1.5pt, color=teal!85, mark=, mark options={fill=teal!85, scale=0.8}]}
\addlegendentry{Multimodal}

\addlegendimage{line width=1.5pt, color=purple!75, mark=, mark options={fill=purple!75, scale=0.8}}
\addlegendentry{Multimodal + Text-only}

\addlegendimage{dashed, line width=1.5pt, color=black!}
\addlegendentry{Base LLM performance}

\end{axis}
\end{tikzpicture}
\vspace{0.3cm}

\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=7cm,
    height=4.0cm,
    ylabel={Performance},
    ylabel near ticks,
    title={Multimodal performance (VQAv2\textsubscript{Eus})},
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[line width=1.5pt, color=teal!85, mark=*, mark options={fill=teal!85, scale=0.8}] coordinates {
    (0, 0.45) (20, 0.59) (80, 0.62) (100, 0.61)
};
\addplot[line width=1.5pt, color=purple!75, mark=*, mark options={fill=purple!75, scale=0.8}] coordinates {
    (0, 0.39) (20, 0.59) (80, 0.61) (100, 0.56)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=7cm,
    height=4.0cm,
    title={Text-only performance (BertaQA local)},
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[dashed, line width=2pt, color=black!70] coordinates {(0, 0.66) (100, 0.66)};
\addplot[line width=1.5pt, color=teal!85, mark=*, mark options={fill=teal!85, scale=0.8}] coordinates {
    (0, 0.52) (20, 0.51) (80, 0.52) (100, 0.53)

};
\addplot[line width=1.5pt, color=purple!75, mark=*, mark options={fill=purple!75, scale=0.8}] coordinates {
    (0, 0.60) (20, 0.55) (80, 0.53) (100, 0.61)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{tikzpicture}[overlay, remember picture]
\fill[purple!35!white] (0.1, 0.5) rectangle (0.7, 2.9);
\node[rotate=90, anchor=center] at (0.4, 1.7) {\large \textbf{Latxa}};
\end{tikzpicture}
\vspace{0.7cm}

\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Basque Multimodal Data \%},
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=7cm,
    height=4.0cm,
    xlabel near ticks,
    ylabel={Performance},
    ylabel near ticks,
    title style={at={(0.5,0.95)}, anchor=south},
]
\addplot[line width=1.5pt, color=teal!85, mark=*, mark options={fill=teal!85, scale=0.8}] coordinates {
    (0, 0.24) (20, 0.56) (80, 0.59) (100, 0.59)
};
\addplot[line width=1.5pt, color=purple!75, mark=*, mark options={fill=purple!75, scale=0.8}] coordinates {
    (0, 0.50) (20, 0.57) (80, 0.61) (100, 0.60)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Basque Multimodal Data \%},
    xmin=-5, xmax=105,
    ymin=0, ymax=1.0,
    xtick={0, 20, 40, 60, 80, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    grid=major,
    width=7cm,
    height=4.0cm,
    xlabel near ticks,
]
\addplot[dashed, line width=2pt, color=black!70] coordinates {(0, 0.45) (100, 0.45)};
\addplot[line width=1.5pt, color=teal!85, mark=*, mark options={fill=teal!85, scale=0.8}] coordinates {
    (0, 0.40) (20, 0.39) (80, 0.41) (100, 0.38)
};
\addplot[line width=1.5pt, color=purple!75, mark=*, mark options={fill=purple!75, scale=0.8}] coordinates {
    (0, 0.41) (20, 0.43) (80, 0.43) (100, 0.41)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{tikzpicture}[overlay, remember picture]
\fill[blue!35!white] (0.1, 1.1) rectangle (0.7, 3.5);
\node[rotate=90, anchor=center] at (0.4, 2.3) {\large \textbf{Llama}};
\end{tikzpicture}

\caption{Accuracy across Basque multimodal (left) and text-only (right) benchmarks of Latxa-based (top row) and Llama-based (bottom row) MLLMs  trained with different percentages of Basque Multimodal Instruction Data. The models are evaluated on the English (original) and Basque (translated) versions.}
\label{fig:performance_benchmark_text_only}
\end{figure*}

